miniKanren as a Tool for Symbolic Computation in Python

In this article, we give a brief overview of the current state and future potential of symbolic computation within the Python statistical modeling and machine learning community. We detail the use of miniKanren as an underlying framework for term rewriting and symbolic mathematics, as well as its ability to orchestrate the use of existing Python libraries. We also discuss the relevance and potential of relational programming for implementing more robust, portable, domain-specific "math-level" optimizations--with a slight focus on Bayesian modeling. Finally, we describe the work going forward and raise some questions regarding potential cross-overs between statistical modeling and programming language theory.

==> math-commands.tex <==
%
% Basic math commands
%
% brandonwillard@gmail.com
% (some material originally borrowed from Thomas Minka)
%
\RequirePackage{mathtools}

\newtheorem{Exa}{Example}

%\usepackage{xifthen}
\let\D\relax
\DeclareMathOperator*{\D}{D}
\let\H\relax
\DeclareMathOperator*{\H}{H}
\DeclareMathOperator*{\prox}{prox}
%\newcommand{\prox}[2] {
%  \ensuremath{
%    \operatornamewithlimits{prox}_{#1}\ifthenelse{\equal{#2}{}}{}{\left(#2\right)}
%  }
%}
\newcommand*{\moreau}[2]{
  \ensuremath{
    {#2}^{
    \ifx&#1&\empty 1 \else #1 \fi
    }
    %{#2}^{\ifthenelse{\equal{#1}{}}{1}{#1}}
  }
}

\newcommand*{\jac}[1]{
  \ensuremath{ \operatornamewithlimits{J}_{#1}
  }
}


\DeclareMathOperator{\dom}{dom}
\newcommand{\var}{{\rm var}}
\newcommand{\Tr}{^{\rm T}}
\newcommand{\rmlog}{\rm log}
\newcommand{\vtrans}[2]{{#1}^{(#2)}}
\newcommand{\kron}{\otimes}
\newcommand{\schur}[2]{({#1} | {#2})}
\newcommand{\schurdet}[2]{\left| ({#1} | {#2}) \right|}
\newcommand{\had}{\circ}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\invdiag}{\diag^{-1}}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\nullsp}{null}
\DeclareMathOperator{\tr}{tr}
\renewcommand{\vec}{\operatorname{vec}}
\DeclareMathOperator{\vech}{vech}
\renewcommand{\det}[1]{\left| #1 \right|}
\newcommand{\pdet}[1]{\left| #1 \right|_{+}}
\newcommand{\pinv}[1]{#1^{+}}
\DeclareMathOperator{\erf}{erf}
\newcommand{\hypergeom}[2]{\operatorname{{}_{#1}F_{#2}}}

% boldface characters
\renewcommand{\a}{{\bf a}}
\renewcommand{\b}{{\bf b}}
\renewcommand{\c}{{\bf c}}
\renewcommand{\d}{{\rm d}}  % for derivatives
\newcommand{\e}{{\bf e}}
\newcommand{\f}{{\bf f}}
\newcommand{\g}{{\bf g}}
\newcommand{\h}{{\bf h}}
%\newcommand{\k}{{\bf k}}
% in Latex2e this must be renewcommand
\renewcommand{\k}{{\bf k}}
\newcommand{\m}{{\bf m}}
\newcommand{\n}{{\bf n}}
\renewcommand{\o}{{\bf o}}
\newcommand{\p}{{\bf p}}
%\newcommand{\q}{{\bf q}}
\renewcommand{\r}{{\bf r}}
\newcommand{\s}{{\bf s}}
\renewcommand{\t}{{\bf t}}
\renewcommand{\u}{{\bf u}}
\renewcommand{\v}{{\bf v}}
\newcommand{\w}{{\bf w}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
%\newcommand{\z}{{\bf z}}
\newcommand{\A}{{\bf A}}
\newcommand{\B}{{\bf B}}
%\newcommand{\C}{{\bf C}}
%\newcommand{\D}{{\bf D}}
\newcommand{\E}{{\bf E}}
\newcommand{\F}{{\bf F}}
%\newcommand{\G}{{\bf G}}
%\renewcommand{\H}{{\bf H}}
\newcommand{\I}{{\bf I}}
\newcommand{\J}{{\bf J}}
\newcommand{\K}{{\bf K}}
%\renewcommand{\L}{{\bf L}}
\newcommand{\M}{{\bf M}}
\newcommand{\Nor}{{\cal N}}  % for normal density
%\newcommand{\N}{{\bf N}}
\renewcommand{\O}{{\bf O}}
\renewcommand{\P}{{\bf P}}
\newcommand{\Q}{{\bf Q}}
\newcommand{\R}{{\bf R}}
\renewcommand{\S}{{\bf S}}
\newcommand{\T}{{\bf T}}
%\newcommand{\U}{{\bf U}}
\newcommand{\V}{{\bf V}}
\newcommand{\W}{{\bf W}}
\newcommand{\X}{{\bf X}}
\newcommand{\Y}{{\bf Y}}
\newcommand{\Z}{{\bf Z}}

\renewcommand{\Re}{{\mathbb{R}}}

% this is for latex 2.09
% unfortunately, the result is slanted - use Latex2e instead
%\newcommand{\bfLambda}{\mbox{\boldmath$\Lambda$}}
% this is for Latex2e
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}

% Yuan Qi's boldsymbol
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
%\newcommand{\Beta}{\boldsymbol{\eta}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bnabla}{\boldsymbol{\nabla}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bLambda}{\mathbf{\Lambda}}

\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}

\newcommand{\bgamma}{\mathbf{\gamma}}
\newcommand{\bGamma}{\mathbf{\Gamma}}

\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bPsi}{\mathbf{\Psi}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\newcommand{\1}{{\bf 1}}
\newcommand{\0}{{\bf 0}}

%\newcommand{\comment}[1]{}

\newcommand{\bs}{\backslash}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\notS}{{\backslash S}}
\newcommand{\nots}{{\backslash s}}
\newcommand{\noti}{{\backslash i}}
\newcommand{\notj}{{\backslash j}}
\newcommand{\nott}{\backslash t}
\newcommand{\notone}{{\backslash 1}}
\newcommand{\nottp}{\backslash t+1}
% \newcommand{\notz}{\backslash z}

\newcommand{\notk}{{^{\backslash k}}}
%\newcommand{\noti}{{^{\backslash i}}}
\newcommand{\notij}{{^{\backslash i,j}}}
\newcommand{\notg}{{^{\backslash g}}}
\newcommand{\wnoti}{{_{\w}^{\backslash i}}}
\newcommand{\wnotg}{{_{\w}^{\backslash g}}}
\newcommand{\vnotij}{{_{\v}^{\backslash i,j}}}
\newcommand{\vnotg}{{_{\v}^{\backslash g}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\quart}{\frac{1}{4}}
\newcommand{\msgb}{m_{t \leftarrow t+1}}
\newcommand{\msgf}{m_{t \rightarrow t+1}}
\newcommand{\msgfp}{m_{t-1 \rightarrow t}}

\newcommand{\proj}[1]{\operatorname{proj}\negmedspace\left[#1\right]}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\DeclareMathOperator{\dif}{d}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

\DeclareMathOperator{\N}{N}

\newcommand{\Rbar}{ \overline{\R} }
\newcommand{\sgn}{\mathop{\mathrm{sgn}}}

\newcommand{\vnorm}[1]{\left|\left|#1\right|\right|}
\newcommand{\enorm}[1]{\Vert #1 \Vert_2}

%\newcommand{\norm}{\mathcal{N}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cK}{\mathcal{K}}

\newcommand{\tN}{\tilde{N}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tF}{\tilde{F}}

\newcommand{\bx}{{\bf x}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\bX}{{\bf X}}
\newcommand{\by}{{\bf y}}
\newcommand{\IG}{\mathcal{IG}}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\lhat}[1][i]{\hat\lambda_{#1}^{-1(g)}}
\newcommand{\what}[1][j]{\hat\omega_{#1}^{-1(g)}}
\newcommand{\bone}{{\bf 1}}
\newcommand{\Li}{\hat\Lambda^{-1(g)}}
\newcommand{\Oi}{\hat\Omega^{-1(g)}}
\newcommand{\iid}{\stackrel{\mathrm{iid}}{\sim}}
\newcommand{\iidp}{\stackrel{\mathrm{P}}{=}}
\newcommand{\iidd}{\stackrel{\mathrm{D}}{=}}
% NOTE: requires mathtools package
\newcommand{\defeq}{\coloneqq}

%\newtheorem{theorem}{\bf Theorem}
%\newtheorem{Proof}{Proof}
%\newtheorem{Def}{Definition}
%\numberwithin{Def}{section}
%\newtheorem{remark}{\bf Remark}
%\newtheorem{Qes}{Question}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{\bf Lemma}
%\newtheorem{Cor}{\bf Corollary}
%\numberwithin{Cor}{section}
%\newtheorem{Eq}{Equation}[section]

